Multi-view Tracking Using Weakly Supervised Human Motion Prediction

Multi-view approaches to people-tracking have the potential to better handle occlusions than single-view ones in crowded scenes. They often rely on the tracking-by-detection paradigm, which involves detecting people first and then connecting the detections. In this paper, we argue that an even more effective approach is to predict people motion over time and infer people's presence in individual frames from these. This enables to enforce consistency both over time and across views of a single temporal frame. We validate our approach on the PETS2009 and WILDTRACK datasets and demonstrate that it outperforms state-of-the-art methods.

==> figs/supp_nb_views.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[h]
    \begin{center}
    %   \centering\includegraphics[width=0.80\textwidth]{./figs/archi_global_3.png}
    \centering\includegraphics[width=1\linewidth]{images/supp_nv_views_bar.png}
    \end{center}
    % need to be reworded copy from 2018 paper
    \caption{\textbf{Effect of the number of views on MODA}. We use the WILDTRACK dataset to evaluate the effect of having multiple view on the detection accuracy measured using MODA.
    The accuracy increase steadily with the number of view until it reaches a plateau around 6 views.
    }
    \label{fig:supp_views}
    \end{figure}

==> tex/__latexindent_temp.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

When it comes to tracking multiple people,  tracking-by-detection~\cite{Andriluka08}  has  become a  standard paradidgm and has  proven effective  for many  applications  such  as surveillance  or  sports player tracking.  It involves first detecting  the target  objects in individual  frames,  associating  these  detections  into  short  but  reliable trajectories  known  as  tracklets,  and  then  concatenating  them  into  longer  trajectories~\cite{Long18,Henschel18,Keuper18,Yoon18,Kim18,Maksai19}. The grouping of detections intro full trajectories  can also be formulated as the search for multiple min-cost paths on a graph~\cite{Berclaz11,Wang19f}. \PF{No references past 2019. Should some be added? } More recently,  tracking-by-regression~\cite{X}�has been advocated as a potential alternative. \PF{Describe it briefly here.}

These techniques are highly effective when the detections are good. However, the detection algorithms typically operate on single frames and fail to exploit the fact that we have videos that exhibit time consistency. In other words, if someone is detected in one frame, chances is that they should be detected at a neighboring location in the next frame. \PF{Arguably that's exactly what tracking-by-regression does.} In this paper, we argue we can further increase their robustness by training networks to detect {\it flows of people} across images because this allows us to impose temporal consistency constraints on our detections. 

\PF{Stopped here.}



%Multi-view multi-object tracking aims to estimate trajectories of multiple objects from cameras with different viewpoints. It has been a topic of interest in computer vision for many years and receive more attention in recently, due to the superiority in handling occlusions which is often difficult for single-view tracking approaches~\cite{Maksai17,Maksai19,Wang16a}.  In most modern work, the \textit{tracking-by-detection} paradigm is adopted as the golden standard. It divides the tracking process to two parts, with the first step as instance detection for which each object is localized for each frame and the second step is detection association which aligns the instance with the same identity in concessive frames. Even though both parts are essential for a robust tracking system, recent approaches were able to obtain impressive result mainly by improving detection association algorithm, using dynamic programming~\cite{Pirsiavash11}, linear programming~\cite{Jiang07,Berclaz11} or more recent deep neural networks that incorporating appearance similarity~\cite{Kim21}, leveraging object motion model~\cite{} or re-identification property~\cite{}.\WL{To do: add exact reference}

\input{figs/intro}

However, these association techniques require reliable instance detection and poor detection step could entirely ruin the association stage. Most work for object detection purely rely on the single frame information, they typically pre-defined a set of anchors and then learn to fit the estimated bounding box to these anchors~\cite{} frame-by-frame without enforcing these detections to be consistent across concessive video frames. However, in video sequence, there exist such physical constraint that an object cannot teleport in concessive frames, therefore the position of object is consistent over time and such motion consistent is beneficial for detecting objects, as depicted by Fig.~\ref{fig:intro}\WL{we should add a teaser figure here to highlight our motivation}. In this work, we thus focus our attention on the detection part and propose to integrate physical constraint of human motion, that is people cannot teleport and thus the number and location must remain consistent in concessive frames. We thus directly enforce such constraint in a novel detection pipeline which shows superior performance in detecting moving objects in video sequence.

Our model is able to achieve temporally consistent object detection that directly enforcing human motion prior into the detection network. Furthermore, our model does not require any additional annotation and directly generate human motion flow in a weakly supervised manner, with only detection annotation. \WL{It is weakly supervised or self-supervised? I think it should be self-supervision among video frames.} The proposed detection model, along with the modification to existing association algorithm to leverage human flow lead to a novel tracking system that consistently outperform state-of-the-art multi-view multi-object tracking approaches in three benchmark datasets. \WL{add more details, what we do and why it is good}

The contribution of our work is a novel detection model that leverages people motion priors and therefore {\it motion-aware}. Our model directly leverage temporal consistency using self-supervision among video frames and thus does not require extra annotation cost. Furthermore, our approach is able to fusing information from different cameras and remain spatial consistency for human position from different viewpoints.

The rest of the paper is organized as follows. We first briefly discuss recent works on human motion modeling and multi-object tracking and compare the difference between previous work and our approach in Section \ref{sec:related}.  We then introduce a novel formulation to directly model human motions in concessive video frames inside the object detector that can consistently improve the detection performance in Section~\ref{sec:approach}.
In Section \ref{sec:expe}, we  show that our approach is compatible with current detection association approaches which consistently outperforms state-of-the-art work in three challenging multi-view multi-object benchmark datasets by a large margin. Lastly, we summarize our work and discuss potential future perspectives in Section \ref{sec:conclusion}.


% \begin{itemize}
%     \item Probabilistic human flow model
%     \begin{itemize}
%         \item weakly supervised people flow
%         \item Temporal consistency through architecture?
%         \item View aggregation mechanism
%         \item Spatial aggregation multi camera fusion
%         \item 
%     \end{itemize}
    
    
%     \item KSP with flow
% \end{itemize}

